On the use of Silver Standard Data for Zero-shot Classification Tasks in Information Extraction

The superior performance of supervised classification methods in the information extraction (IE) area heavily relies on a large amount of gold standard data. Recent zero-shot classification methods converted the task to other NLP tasks (e.g., textual entailment) and used off-the-shelf models of these NLP tasks to directly perform inference on the test data without using a large amount of IE annotation data. A potentially valuable by-product of these methods is the large-scale silver standard data, i.e., pseudo-labeled data by the off-the-shelf models of other NLP tasks. However, there is no further investigation into the use of these data. In this paper, we propose a new framework, Clean-LaVe, which aims to utilize silver standard data to enhance the zero-shot performance. Clean-LaVe includes four phases: (1) Obtaining silver data; (2) Identifying relatively clean data from silver data; (3) Finetuning the off-the-shelf model using clean data; (4) Inference on the test data. The experimental results show that Clean-LaVe can outperform the baseline by 5% and 6% on TACRED and Wiki80 dataset in the zero-shot relation classification task, and by 3%-7% on Smile (Korean and Polish) in the zero-shot cross-lingual relation classification task, and by 8% on ACE05-E+ in the zero-shot event argument classification task. The code is share in https://github.com/wjw136/Clean_LaVe.git.

==> abstract.tex <==
\begin{abstract}
The superior performance of supervised relation extraction (RE) methods heavily relies on a large amount of gold standard data. 
Recent zero-shot relation extraction methods converted the RE task to other NLP tasks and used off-the-shelf models of these NLP tasks to directly perform inference on the test data without using a large amount of RE annotation data. 
A potentially valuable by-product of these methods is the large-scale silver standard data. 
However, there is no further investigation on the use of potentially valuable silver standard data. 
In this paper, we propose to first detect a small amount of clean data from silver standard data and then use the selected clean data to finetune the pretrained model. 
We then use the finetuned model to infer relation types.
% We also propose a class sampler to prevent unbalanced clean data harming the model. # written_on_abstract_ddl
We also propose a class-Aware clean data detection module to consider class diversity when selecting clean data.
The experimental results show that our method can outperform the baseline by 12\% and 11\% on TACRED and Wiki80 dataset in the zero-shot RE task. By using extra silver standard data of different distributions, the performance can be further improved.
\end{abstract}

==> limitations.tex <==
\section*{Limitations}

\begin{itemize}
\item The performance of our proposed method relies on the quality of silver standard data. Underperforming pretrained models will lead to noisy silver standard data and deteriorate the performance.  
% In addition, the good performance also depends on an efficient clean data detection module. 
% \item \revisezq{We only demonstrate the effectiveness of using clean silver data to improve pretrained models on relation extraction task. Its effects on other NLP tasks need further exploration. }
% \item \revisety{In order to use data cleaning algorithms to select data with high accuracy, We need to annotate a large number of data, which is time-consuming.}
\item It is time-consuming to annotate unlabeled data using an off-the-shelf TE model. 
It takes 3.5 hours and 2.2 hours to annotate the training set of TACRED and Wiki80 respectively. The training time of our method is 1.5 hours. 
% \item \revisezq{We use WikiFact as extra data because the entities are identified. We currently can perform relation classification task but cannot jointly perform entity recognition and relation classification in zero-shot setting. There is still a constraint when utilizing extra data.}
% \item In our proposed method, when training silver data to get its confidence or loss, we train in a fixed-epoch manner because there is no metric to indicate when the training process should stop. However, if we stop training too early or too late, the quality of the clean data deteriorates. Thus, such stop indication needs to be investigated.
\end{itemize}
